Adversary Agnostic Robust Deep Reinforcement Learning

Deep reinforcement learning (DRL) policies have been shown to be deceived by perturbations (e.g., random noise or intensional adversarial attacks) on state observations that appear at test time but are unknown during training. To increase the robustness of DRL policies, previous approaches assume that the knowledge of adversaries can be added into the training process to achieve the corresponding generalization ability on these perturbed observations. However, such an assumption not only makes the robustness improvement more expensive but may also leave a model less effective to other kinds of attacks in the wild. In contrast, we propose an adversary agnostic robust DRL paradigm that does not require learning from adversaries. To this end, we first theoretically derive that robustness could indeed be achieved independently of the adversaries based on a policy distillation setting. Motivated by this finding, we propose a new policy distillation loss with two terms: 1) a prescription gap maximization loss aiming at simultaneously maximizing the likelihood of the action selected by the teacher policy and the entropy over the remaining actions; 2) a corresponding Jacobian regularization loss that minimizes the magnitude of the gradient with respect to the input state. The theoretical analysis shows that our distillation loss guarantees to increase the prescription gap and the adversarial robustness. Furthermore, experiments on five Atari games firmly verify the superiority of our approach in terms of boosting adversarial robustness compared to other state-of-the-art methods.

==> sections/Bio.tex <==
% \clearpage
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/photo/xinghua}}]{Xinghua Qu}
received the B.S. and  M.S. degrees in Aerospace from Northwestern Polytechnic University in 2014, and Beihang University in 2017, respectively. Currently he is a final year PhD student at the school of computer science and engineering in
Nanyang Technological University. His primary research interest includes machine learning and optimisation.
Recently his research interest mainly focuses on the trustworthy of
reinforcement learning, including adversarial robustness evaluation, adversarial defence
techniques and off-line RL.
\end{IEEEbiography}
% \vspace{-0.4in}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/photo/ong}}]{Yew-Soon Ong}
received his PhD degree on Artificial
Intelligence in complex design from the Computational Engineering and Design Center, University
of Southampton, UK in 2003.  He is a President Chair Professor of Computer Science at Nanyang Technological University (NTU), and
holds the position of Chief Artificial Intelligence Scientist at the Agency for Science, Technology and Research in Singapore. At NTU, he serves as Director of the Singtel-NTU Cognitive \& Artificial Intelligence Joint Lab. His research interest lies in artificial and computational intelligence. He is the founding Editor-in-Chief of the IEEE Transactions on Emerging Topics in Computational Intelligence and AE of IEEE Transactions on Neural Networks \& Learning Systems, the IEEE Transactions on Cybernetics, and others.
\end{IEEEbiography}
% \vspace{-0.4in}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/photo/abhishek}}]{Abhishek Gupta}
received his PhD in Engineering Science from the University of Auckland, New
Zealand, in the year 2014. He graduated with a
Bachelor of Technology degree in the year 2010,
from the National Institute of Technology Rourkela,
India. He currently serves as a Scientist in the
Singapore Institute of Manufacturing Technology
(SIMTech), Agency of Science, Technology and
Research (A*STAR), Singapore. He has diverse
research experience in the field of computational
science, ranging from numerical methods in engineering physics, to topics in computational intelligence. His recent research
interests are in the development of memetic computation for
automated knowledge extraction and transfer across problems in evolutionary
design.
\end{IEEEbiography}
% \vspace{-0.4in}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/photo/sunzhu}}]{Zhu Sun}
received her Ph.D. degree from School of Computer Science and Engineering,
Nanyang Technological University (NTU), Singapore, in 2018. She is a Lecturer/Assistant Professor at the Department of Computing, Macquarie University, Sydney, Australia. Her research interests are mainly focused on designing efficient recommendation algorithms by considering side information. Her research has been published in leading
conferences and journals in related domains (e.g., IJCAI, AAAI, CIKM, 
ACM RecSys and ACM UMAP and IEEE Transactions).
%Currently, she is a researchfellow at School of Electrical and Electronic Engineering, NTU, Singapore.
\end{IEEEbiography}




==> sections/table_2.tex <==
\begin{table*}[h]
    \centering
    \scriptsize
    \addtolength{\tabcolsep}{3.4pt}
    \renewcommand{\arraystretch}{1.4}
	\caption{Comparison of relative robustness measured by $\mathcal{M(\cdot)}$ in Eq.~(\ref{eq:relative_robustness}) based on the results in Table~\ref{table:robustness comparison}. The comparison with previous studies under PGD attack with different PGD iteration $K$.}
	\label{tab:robustness_compare}
	\addtolength{\tabcolsep}{-2.5pt}
    \begin{tabular}{|l|l|lllll|}
    \specialrule{.15em}{.05em}{.05em}
    \multirow{2}{*}{Method} &\multirow{2}{*}{Evaluation Case} &\multicolumn{5}{c|}{\textbf{Atari Games}}\\
    \cline{3-7}
     && Freeway &Bank Hesit &Pong &Boxing &Road Runner\\
    \specialrule{.1em}{.05em}{.05em}
    \multirow{6}{*}{Ours}
    &
    % \rowcolor{maroon!20}
    $\mathcal{M}(\pi_{\theta^S}\text{PGD}(K=4),\pi_{\theta^T})$& $-0.58\%$ &$0.25\%$ & $-3.33\%$ & $-26.05\%$& $-61.12\%$\\
    &
    % \rowcolor{maroon!20}
    $\mathcal{M}(\pi_{\theta^S}\text{PGD}(K=4),\pi_{\theta^S})$& $-0.97\%$ &$-0.49\%$ & $-3.33\%$ & $-1.96\%$& $0.67\%$\\
    &
    % \rowcolor{LightCyan}
    $\mathcal{M}(\pi_{\theta^S}\text{PGD}(K=10),\pi_{\theta^T})$& $-6.62\%$ &$0.71\%$ & $-3.33\%$ & $-23.73\%$& $-61.52\%$\\
    &
    % \rowcolor{LightCyan}
    $\mathcal{M}(\pi_{\theta^S}\text{PGD}(K=10),\pi_{\theta^S})$& $-6.98\%$ &$-0.04\%$ & $-3.33\%$ & $1.12\%$& $0.37\%$\\
    &$\mathcal{M}(\pi_{\theta^S}\text{PGD}(K=20),\pi_{\theta^T})$& $-3.87\%$ &$0.74\%$ & $-4.29\%$ & $-26.05\%$& $-65.85\%$\\
    &$\mathcal{M}(\pi_{\theta^S}\text{PGD}(K=20),\pi_{\theta^S})$& $-4.25\%$ & $0.00\%$& $-4.29\%$ & $-1.96\%$ & $-11.57\%$\\
    \specialrule{.1em}{.05em}{.05em}
    \multirow{2}{*}{\cite{fischer2019online} }
    &
    % \rowcolor{maroon!20}
    $\mathcal{M}(\text{RS-DQN PGD} (K=4), \text{DQN})$ & $-1.42\%$ & $-14.11\%$ & $-10.24\%$ & $-46.93\%$ & $-38.83\%$\\
    &
    % \rowcolor{maroon!20}
    $\mathcal{M}(\text{RS-DQN PGD} (K=4), \text{RS-DQN})$ & $-1.21\%$ & $-19.87\%$ & $-8.11\%$ & $-36.94\%$ & $-52.48\%$\\
    \specialrule{.1em}{.05em}{.05em}
    \multirow{2}{*}{\cite{zhang2020robust}}
    &
    % \rowcolor{LightCyan}
    $\mathcal{M}(\text{SA-DQN PGD} (K=10), \text{DQN})$ & $-7.72\%$ & $-20.24\%$ & $-2.90\%$ & NA & $-58.64\%$\\
    &
    % \rowcolor{LightCyan}
    $\mathcal{M}(\text{SA-DQN PGD} (K=10), \text{SA-DQN})$& $-1.65\%$ & $0.21\%$ & $-4.29\%$ & NA & $0.71\%$\\
    \specialrule{.15em}{.05em}{.05em}
    \end{tabular}
    \label{table:relative_robustness comparison}
    \vspace{-0.2in}
\end{table*}
